Linking Vision and Multi-Agent Communication through Visible Light Communication using Event Cameras

Various robots, rovers, drones, and other agents of mass-produced products are expected to encounter scenes where they intersect and collaborate in the near future. In such multi-agent systems, individual identification and communication play crucial roles. In this paper, we explore camera-based visible light communication using event cameras to tackle this problem. An event camera captures the events occurring in regions with changes in brightness and can be utilized as a receiver for visible light communication, leveraging its high temporal resolution. Generally, agents with identical appearances in mass-produced products are visually indistinguishable when using conventional CMOS cameras. Therefore, linking visual information with information acquired through conventional radio communication is challenging. We empirically demonstrate the advantages of a visible light communication system employing event cameras and LEDs for visual individual identification over conventional CMOS cameras with ArUco marker recognition. In the simulation, we also verified scenarios where our event camera-based visible light communication outperforms conventional radio communication in situations with visually indistinguishable multi-agents. Finally, our newly implemented multi-agent system verifies its functionality through physical robot experiments.

==> 3_1_fig2_explanation.tex <==
\subsection{Camera-based VLC for multiagent tasks} \label {approach_task}
When introducing event cameras into a multi-agent system for VLC, a comparison with existing communication technologies is presented in Fig.~\ref{fig:linkingvisualcomm}. Identifying agents using RGB cameras in environments where self-location is not feasible is challenging. As shown in Fig.~\ref{fig:linkingvisualcomm} (a), distinguishing other agents using RGB cameras is not possible, and even if the signals obtained through radio communication are associated with IDs, linking them to individual agents visually is difficult. In other words, it becomes a situation where it is unclear which agent is transmitting which communication information based on the acquired communication data. In contrast, when using VLC, communication is only possible with visible agents, and communication with agents behind walls is impossible. However, communication and visual information are linked regarding visible other agents, allowing an understanding of the information conveyed by visible agents. When using a single photodiode as Rx, as mentioned in Table~\ref{comparevlc}, separating the signals of interest is impossible. Therefore, when receiving signals from multiple agents, it is not possible to determine which agent they came from (Fig.~\ref{fig:linkingvisualcomm}(b)). On the other hand, in the case of VLC using event cameras, signal information can be obtained as visual information within the visible range, allowing signal separation and the advantage of linking the communication content of each agent to the respective agent. In other words, it becomes possible to understand what the left agent is saying and what the right agent is saying.


By processing visual information while identifying individual IDs, it is believed that there are tasks and situations in which a multi-agent system can gain an advantage. First, this is the case when communication information serves to grasp spatial relationships. In other words, in tasks where agents with limited FOV, for example, need to communicate what they currently see to understand the surrounding situation, the linkage between the aforementioned visual information and communication information becomes crucial. Furthermore, in tasks requiring spatial fine-tuning with neighboring agents, such as group arrangements, it is possible to increase the success rate of the task by understanding what information neighboring agents are conveying that cannot be sufficiently grasped by visual information alone. It is also conceivable that VLC signals, which have limitations compared to radio communication, can be used inversely to avoid acquiring unnecessary information, making them effective when acting in a distributed manner.

